A frequency-constrained geometric Pontryagin maximum principle on matrix Lie groups

In this article we present a geometric discrete-time Pontryagin maximum principle (PMP) on matrix Lie groups that incorporates frequency constraints on the controls in addition to pointwise constraints on the states and control actions directly at the stage of the problem formulation. This PMP gives first order necessary conditions for optimality, and leads to two-point boundary value problems that may be solved by shooting techniques to arrive at optimal trajectories. We validate our theoretical results with a numerical experiment on the attitude control of a spacecraft on the Lie group SO(3).

==> Makefile <==
# Make file for easy build and cleanup
REQ = freqKPMP.tex
FILENAME = $(REQ:.tex=)
DEP = kpmp_defs.sty introduction.tex \
	  main_result.tex problem.tex proof.tex \
	  references.bib simulations.tex fallback.tex
GOAL = $(REQ:.tex=.pdf)


.PHONY: clean show force-clean pull transfer

$(GOAL): $(REQ) $(DEP)
	latexmk -silent -time -pdf $(FILENAME)
	make clean

show: $(REQ) $(DEP)
	latexmk -time -pdf $(FILENAME)
	make clean

clean:
	latexmk -c -time $(FILENAME)

force-clean:
	latexmk -C -time $(FILENAME)


